Advancing Semantic Caching for LLMs with Domain-Specific Embeddings and Synthetic Data

This report investigates enhancing semantic caching effectiveness by employing specialized, fine-tuned embedding models. Semantic caching relies on embedding similarity rather than exact key matching, presenting unique challenges in balancing precision, query latency, and computational efficiency. We propose leveraging smaller, domain-specific embedding models, fine-tuned with targeted real-world and synthetically generated datasets. Our empirical evaluations demonstrate that compact embedding models fine-tuned for just one epoch on specialized datasets significantly surpass both state-of-the-art open-source and proprietary alternatives in precision and recall. Moreover, we introduce a novel synthetic data generation pipeline for the semantic cache that mitigates the challenge of limited domain-specific annotated data, further boosting embedding performance. Our approach effectively balances computational overhead and accuracy, establishing a viable and efficient strategy for practical semantic caching implementations.

==> graphs/catastrophic-forgetting-solution.tex <==
\begin{adjustbox}{width=\textwidth}
% \begin{center}
\begin{tikzpicture}
    \begin{axis}[
        % width=0.45\textwidth,
        % height=0.45\textwidth,
        width=\textwidth,
        height=0.7\textwidth,
        ybar=0pt,
        bar width=10pt,
        enlarge x limits=0.1,
        xlabel={Metric},
        ylabel={Score},
        ymin=0.0,
        ymax=1.05,
        symbolic x coords={Precision, Recall, F1 Score, Accuracy, Avg. Precision},
        xtick=data,
        xticklabel style={
          rotate=30,
          anchor=east,
          font=\small
        },
        ytick scale label code/.code={},
        nodes near coords,
        every node near coord/.append style={
          font=\tiny,
          yshift=1pt
        },
        legend style={
          at={(-0.5,1.05)},
          anchor=south,
          font=\small,
          legend columns=2,
          /tikz/every even column/.append style={column sep=1ex}
        },
        legend cell align={left},
        tick label style={font=\scriptsize},
        label style={font=\small},
        axis on top,
        grid=both,
        grid style={dashed, gray!30}
      ]

      \addplot [fill=blue!70] coordinates {
        (Precision, 0.82)
        (Recall, 0.90)
        (F1 Score, 0.86)
        (Accuracy, 0.85)
        (Avg. Precision, 0.92)
      };

      \addplot [fill=blue!30] coordinates {
        (Precision, 0.78)
        (Recall, 0.92)
        (F1 Score, 0.84)
        (Accuracy, 0.83)
        (Avg. Precision, 0.92)
      };

      \legend{Redis-ModernBert, ModernBert-Base (base)}
    \end{axis}
  \end{tikzpicture}
% \end{center}
\end{adjustbox}

==> graphs/catestrophic-figure-problem.tex <==
\begin{adjustbox}{width=\textwidth}
% \begin{center}
\begin{tikzpicture}
    \begin{axis}[
        % width=\columnwidth,
        % height=0.5\columnwidth,
        % width=6cm,
        % height=4cm,
        width=\textwidth,
        height=0.7\textwidth,
        ybar=0pt,
        bar width=12pt,
        enlarge x limits=0.1,
        xlabel={Metric},
        ylabel={Score},
        ymin=0.0,
        ymax=1.05,
        symbolic x coords={Precision, Recall, F1 Score, Accuracy, Avg. Precision},
        xtick=data,
        xticklabel style={
          rotate=30,
          anchor=east,
          font=\small
        },
        nodes near coords,
        every node near coord/.append style={
          font=\tiny,
          yshift=2pt
        },
        % legend style={
        %   at={(0.5,1.15)},
        %   anchor=south,
        %   font=\small,
        %   legend columns=2,
        %   /tikz/every even column/.append style={column sep=1ex}
        % },
        % legend cell align={left},
        tick label style={font=\scriptsize},
        label style={font=\small},
        axis on top,
        grid=both,
        grid style={dashed, gray!30}
    ]

    % Redis-Finetuned-gte-modernbert-base (Ours)
    \addplot [fill=blue!70] coordinates {
        (Precision, 0.70)
        (Recall, 0.85)
        (F1 Score, 0.77)
        (Accuracy, 0.74)
        (Avg. Precision, 0.82)
    };

    % Base-gte-modernbert-base
    \addplot [fill=blue!30] coordinates {
        (Precision, 0.78)
        (Recall, 0.92)
        (F1 Score, 0.84)
        (Accuracy, 0.83)
        (Avg. Precision, 0.92)
    };

    % \legend{Redis-Finetuned-gte-modernbert-base (Our), Base-gte-modernbert-base}
    \end{axis}
\end{tikzpicture}
% \end{center}
\end{adjustbox}
